Deep Learning for End-to-End Atrial Fibrillation Recurrence Estimation

Left atrium shape has been shown to be an independent predictor of recurrence after atrial fibrillation (AF) ablation. Shape-based representation is imperative to such an estimation process, where correspondence-based representation offers the most flexibility and ease-of-computation for population-level shape statistics. Nonetheless, population-level shape representations in the form of image segmentation and correspondence models derived from cardiac MRI require significant human resources with sufficient anatomy-specific expertise. In this paper, we propose a machine learning approach that uses deep networks to estimate AF recurrence by predicting shape descriptors directly from MRI images, with NO image pre-processing involved. We also propose a novel data augmentation scheme to effectively train a deep network in a limited training data setting. We compare this new method of estimating shape descriptors from images with the state-of-the-art correspondence-based shape modeling that requires image segmentation and correspondence optimization. Results show that the proposed method and the current state-of-the-art produce statistically similar outcomes on AF recurrence, eliminating the need for expensive pre-processing pipelines and associated human labor.

==> README <==
file: README

Writing a CinC Paper Using LaTeX

George Moody (george@mit.edu)
Last revised: 20 February 2012

This directory contains the CinC Author's Kit for preparing papers in
PDF format using LaTeX.  The following files are included:

 README		this file

 balance.sty	LaTeX macro for equalizing column length

 cinc.cls	CinC style file

 cinc.bst	CinC bibliography style file

 template.tex	generic template for a paper (LaTeX source)

 template.pdf	formatted version of template.tex

 refs.bib	sample BibTeX bibliography file

 Makefile	rules for generating template.pdf using a 'make' utility

 pdftex.cfg	needed if using an old (pre-2002) version of pdflatex (see
		the note at the end of this file)

 example1, example2
		directories containing two complete sample papers, including
		figures and bibliography files

 makebst	directory containing files needed to generate cinc.bst


INSTALLATION

This kit can be used with any reasonably modern (September, 1994 or later)
version of LaTeX, a dialect of Donald Knuth's TeX software for typesetting.

If you don't already have LaTeX on your computer, download and install it now.
We recommend:

    TeX Live (http://www.tug.org/texlive/) for Linux or other Unix
    MacTeX (http://www.tug.org/mactex/) for Mac OS X
    proTeXt (http://www.tug.org/protext/) for MS Windows

All are free and include everything needed other than the CinC-specific files
included in this author's kit.

To install the files provided in this directory, do one of the following:

* Copy cinc.cls and cinc.bst to the directory that will contain your
  paper.

   -- or --

* Copy them to the standard locations for files of these types.  You may need
  to run texhash or mktexlsr afterwards, so that LaTeX and BibTeX can find
  these files.

If your installation of LaTeX doesn't include balance.sty, copy balance.sty
from this directory into the same location where you copied cinc.cls.

The instructions below assume that you will use pdflatex to process your
paper and to create a PDF file from it. The recommended TeX distributions
mentioned above, and most others, include pdflatex. If you don't use pdflatex,
use extra care to be sure that the page size and margins in your final PDF are
correct; see the Appendix for details.


FORMATTING THE EXAMPLES (OPTIONAL)

The use of these files is best illustrated by the included sample papers
(example1/example1.tex and example2/example2.tex), which are accompanied by
sets of PDF (.pdf), PostScript (.ps), and encapsulated PostScript (.eps)
figures in example*/figures/, and by BibTeX bibliography (.bib) files in
example*/bib/, all of which are referenced in the papers.  To format the sample
papers:

1. Install cinc.cls and cinc.bst by copying them from this directory into the
   example directories, or into the standard locations.

2. Enter the example1 directory and do the following:
	pdflatex example1   [creates example1.aux, needed by bibtex]
	bibtex example1	    [creates example1.bbl, needed by pdflatex]
	pdflatex example1   [merges references]
	pdflatex example1   [produces final PDF with correct citation numbers]

The multiple runs of pdflatex are needed to prepare data for bibtex and
then to resolve the cross-references. These steps produce example1.pdf (and
several temporary files that can be removed).

The 'Makefile' included in each directory can be used by a 'make' utility
to automate these steps.

A similar procedure can be used to format example2.tex, which illustrates
other features of the CinC style files.


WRITING YOUR PAPER

Make a copy of the generic template (template.tex). The instructions below
assume that you have saved your copy of the template as a file named paper.tex,
into which you can type your paper.

Please use the example files provided as models for your own papers. 
All references should be entered in BibTeX (.bib) database files (see the
samples in the example*/bib directories).  In order to conform to the layout
instructions, please check your final version against the example layout
provided (http://www.cinc.org/authors_kit/papers/example_layout.pdf).  Please
double-check that you have followed these rules:

 1. The title of the paper should not end with a "."

 2. List the authors of the paper in the form:
	Albert B Johnson, Charles X Anderson
    Do not use "." after initials, and do not use the word "and" before the
    name of the last author.  Since CinC is an English-language publication,
    and to ensure that your paper will be indexed correctly, follow the
    English-language convention for name order: given name(s) first, family
    names (surnames) last.

 3. List the authors' institutions within the \author statement.  Use
    superscripted numerals to identify the affiliations of each author if
    necessary.  Use \\ to force a line break if needed, and use \mbox{}\\ to
    create a blank line between the  authors' names and their institutions.
    For example:

     \author{Hans~A~Kestler$^{1,2}$, Friedhelm~Schwenker$^1$, G~Hafner$^1$,
      Vinzenz~Hombach$^2$, G{\"u}nter~Palm$^1$, Martin~H{\"o}her$^2$ \\
      \mbox{}\\
      $^1$Neural Information Processing, University of Ulm, Germany \\
      $^2$Medicine II -- Cardiology, University Hospital Ulm, Germany}

 4. Inside table environments, place the \caption at the beginning to insure
    that the table legend appears above the table.  Inside figure environments,
    the \caption goes at the end, so that it appears below the figure.	

 5. To create two equal-length columns on the last page, first identify what
    portion of your paper would be included in the first column on the
    last page, then insert the command
	\balance
    anywhere within this portion of text, and reformat.  (This works because
    cinc.cls now includes the standard 'balance.sty' package.  Thanks to
    Erik Bojorges for this suggestion.)


FORMATTING YOUR PAPER

You must submit the LaTeX source for your paper together with any other files
needed to produce a copy of your paper, such as files containing figures,
tables, and references.  Collect them together in a zip file to upload to
the paper collection site.

Before submitting the zip file, test that it is complete and verify that the
files within it produce a properly formatted paper of no more than 4 pages.
Do this by making a test PDF from the contents of the zip file.

You must submit your paper in PDF format (other formats, such as LaTeX
source, DVI, and PostScript, cannot be accepted).  There are several ways to
generate a PDF from LaTeX sources; the recommended method is described below.
The instructions below assume that you have composed your paper in a file
called paper.tex (substitute the name of your file in the commands below,
omitting the .tex suffix).

  1.  Run these commands:
	pdflatex paper
	bibtex paper
	pdflatex paper
	pdflatex paper
  2. If there were any errors or warnings, make any necessary corrections
     and repeat step 1.  Use a PDF viewer (such as Acrobat, xpdf, or a
     recent copy of GhostScript) to view paper.pdf, and correct any
     formatting errors.

If you cannot use pdflatex, an alternative method is described in the Appendix.


SUBMITTING YOUR PAPER

You must submit your paper electronically (paper copies are no longer necessary
or accepted).  Instructions on submitting your paper using your web
browser are included in the CinC Author's Kit.

The Editor will be available during the poster session to answer questions and
give advice. It would be helpful if you bring a single printed copy of your
paper with you, which the Editor may mark and will give back to you.


PRINTING YOUR TEST PDF

Most PDF viewing software can also be used to print PDF files.  If you use
Adobe Acrobat, Distiller, or Reader, choose Page Scaling: None and uncheck Auto
Rotate and Center in the Print dialog; this ensures that your paper will be
printed at the same scale and with the same top and left margins as will be
used in the published Proceedings.  Copies printed on A4 paper will not be
centered on the page, but they should be readable.

You may use color in figures, but print your paper on a black-and-white
printer and be sure that your figures are still legible.  The proceedings
are published in printed form (black-and-white only) as well as on CD-ROMs and
on-line (in color).  It's important that readers of the printed proceedings be
able to see your figures as you intended.

_______________________________________________________________________________

ACKNOWLEDGEMENTS

The cinc.cls file was originally adapted by Hans Kestler from Peter Nuchter's
IEEEtran2e.cls, which in turn was adapted from IEEEtran.sty by Gerry Murray and
Silvano Balemi.  Bob Throne, Alan Murray, Andrew Sims, George Moody, and Erik
Bojorges contributed feedback, bug fixes, and further improvements.  The
cinc.bst file was created by Hans Kestler and George Moody using Patrick Daly's
makebst generator.  George Moody wrote the generic template.

Your comments, suggestions, questions, and bug reports are welcome;  please
send them to George Moody (george@mit.edu).

_______________________________________________________________________________

APPENDIX

Using latex instead of pdflatex

Use this method only if you cannot use pdflatex.

If you have PostScript figures, note that you can still use pdflatex if you
first convert them to PDF using epstopdf, which is included in your TeX
distribution. Use a command such as:

        epstopdf figure.ps

which creates figure.pdf. 

To make an acceptable PDF without using pdflatex, it is very important to
follow the instructions below precisely. In these instructions, note that "\"
at the end of a line indicates that the command continues on the next line. The
instructions below assume that you have composed your paper in a file called
paper.tex (substitute the name of your file in the commands below, omitting the
.tex suffix).

  1.  Run these commands:
	latex paper
	bibtex paper
	latex paper
	latex paper
  2.  You will now have a .dvi file named paper.dvi.
  3.  Run these commands:
	dvips -Ppdf -t letter -o paper.ps paper.dvi
	ps2pdf -dPDFSETTINGS=/printer -dCompatibilityLevel=1.3 \
	 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true \
	 -sPAPERSIZE=letter paper.ps
      VERY IMPORTANT: Use "letter" in the dvips and ps2pdf commands even
      if your normal paper size is A4, since the Proceedings are printed
      on US letter-sized pages.
  4.  If there were any errors or warnings, make any necessary corrections
      and repeat step 1.  Use Acrobat, xpdf, or GhostScript to view paper.pdf,
      and correct any formatting errors.

Using (very) old versions of pdflatex

If you have installed one of the recommended TeX distributions mentioned above,
this section does not apply to you.

If you use a version of pdflatex older than 1.10 (released in 2002), you may
need to copy pdftex.cfg from this directory into the directory that contains
your paper before formatting it with pdflatex.  Versions 1.10 and later
can get the information contained in pdtex.cfg from \pdf... declarations in
cinc.cls, and versions 1.20a and later completely ignore pdftex.cfg.  The
settings in question define the paper size (8.5 x 11 inches, the size used to
print the proceedings) and the location of the coordinate system origin on the
page.  If your pdflatex needs pdftex.cfg and can't find it, your paper size and
margins may be incorrect.  If you are in doubt, open your PDF file with
GhostScript, xpdf, or Adobe Reader and check the paper size, which should be
8.5 x 11 inches (216 x 279 mm), not 210 x 297 mm as for A4 paper.

